Factors of Transferability for a Generic ConvNet Representation

Evidence is mounting that Convolutional Networks (ConvNets) are the most effective representation learning method for visual recognition tasks. In the common scenario, a ConvNet is trained on a large labeled dataset (source) and the feed-forward units activation of the trained network, at a certain layer of the network, is used as a generic representation of an input image for a task with relatively smaller training set (target). Recent studies have shown this form of representation transfer to be suitable for a wide range of target visual recognition tasks. This paper introduces and investigates several factors affecting the transferability of such representations. It includes parameters for training of the source ConvNet such as its architecture, distribution of the training data, etc. and also the parameters of feature extraction such as layer of the trained ConvNet, dimensionality reduction, etc. Then, by optimizing these factors, we show that significant improvements can be achieved on various (17) visual recognition tasks. We further show that these visual recognition tasks can be categorically ordered based on their distance from the source task such that a correlation between the performance of tasks and their distance from the source task w.r.t. the proposed factors is observed.

==> Conclusion.tex <==
\section{Conclusion and Future Works}
\label{sec:conclusion}

==> network_tableB.tex <==
\pgfplotstableset{NetworkParams/.style ={%
        header=true,
        string type,
        font=\footnotesize,
        column type=l,
        every odd row/.style={
            before row=
        },
        every head row/.style={
            before row={%
              \topline\rowcolor{tableheadcolor}
             &  &            
            \multicolumn{3}{c}{\textbf{Convolutional layers}}
            & 
            \multicolumn{2}{c}{\textbf{FC layers}}
            %% & 
            %% \multicolumn{2}{c}{\textbf{Output layer}}
            \\
            \arrayrulecolor{tableheadcolor} \specialrule{6pt}{0pt}{-6pt} \arrayrulecolor{rulecolor}
            \cmidrule(r){3-5} \cmidrule(r){6-7} %\cmidrule(r){8-9}
            \rowcolor{tableheadcolor}
            },
            after row={\midtopline}
        },
        every last row/.style={
            after row=\bottomline
        },
        columns/network/.style = {column name=\textbf{Network}},
        columns/TotalNum/.style = {column name=$N_T$},
        columns/ConvNum/.style = {column name=\#},
        columns/NumKernels/.style = {column name= $n_l\times n_k$ per
          layer},
        columns/SzKernels/.style = {column name= kernel sizes per
          layer},
        columns/ConvOutDims/.style = {column name= out dim},
        columns/FCNum/.style = {column name=\#},
        columns/FCSize/.style = {column name=$n_h$ per layer},
        columns/OutputType/.style = {column name=function},
        columns/OutputNum/.style = {column name=$n_o$},
        col sep=&,
        row sep=\\
    }
}
\begin{table}
\setlength{\tabcolsep}{2pt}
  \caption{\textbf{Deeper Networks:} Size details of the different ConvNet depths used in our experiments.}
  \label{tab:network_size}
\centering
{\centering
  \pgfplotstabletypeset[NetworkParams]{ 
    network & TotalNum & ConvNum & NumKernels & ConvOutDims & FCNum &
    FCSize %% & OutputType & OutputNum
    \\
    Deep8   & 85M & 5  & (1$\times$64, 1$\times$128, 3$\times$256) &8$\times$8$\times$256& 3 & (4096, 4096, 1000) 
    %% & SoftMax & 1000
    \\
    \midrule
    Deep11  & 86M & 8 &  (1$\times$64, 3$\times$128, 4$\times$256) &8$\times$8$\times$256& 3 & (4096, 4096, 1000) 
    \\
    \midrule
    Deep13  & 86M & 10 & (2$\times$64, 4$\times$128, 4$\times$256) &8$\times$8$\times$256& 3 & (4096, 4096, 1000) 
    \\
    \midrule
    Deep16  & 87M & 13 & (2$\times$64, 5$\times$128, 6$\times$256) &8$\times$8$\times$256& 3 & (4096, 4096, 1000) 
    \\
  }
}
\\[2pt]
\raggedright
{\footnotesize{ 
The description of the notation in the table: $N_T$ is the
  total number of weights parameters in the network, $n_k$ is the
  number of kernels at a convolutional layer, $n_l$ is the number of layers with $n_k$ kernels, and $n_h$ is the number
  of nodes in a fully connected layer. For each network the output
  layer applies a SoftMax function and has 1000 output nodes. The
  networks are ordered w.r.t. their total number of parameters. Note that these networks are re-trained for our experiments and the model might differ from that of \cite{Simonyan14}, for instance we do not use multi-scale input and our input image size is 227x227, we do random cropping as implemented in \texttt{Caffe}, etc.}}
\label{tab:net_sizes_depth}
\end{table}


==> network_tableC.tex <==
\pgfplotstableset{NetworkParams/.style ={%
        header=true,
        string type,
        font=\footnotesize,
        column type=l,
        every odd row/.style={
            before row=
        },
        every head row/.style={
            before row={%
              \topline\rowcolor{tableheadcolor}
             &  &
            \multicolumn{2}{c}{\textbf{Convolutional layers}}
            & 
            \multicolumn{2}{c}{\textbf{FC layers}}
            %% & 
            %% \multicolumn{2}{c}{\textbf{Output layer}}
            \\
            \arrayrulecolor{tableheadcolor} \specialrule{6pt}{0pt}{-6pt} \arrayrulecolor{rulecolor}
            \cmidrule(r){3-4} \cmidrule(r){5-6} %\cmidrule(r){8-9}
            \rowcolor{tableheadcolor}
            },
            after row={\midtopline}
        },
        every last row/.style={
            after row=\bottomline
        },
        columns/network/.style = {column name=\textbf{Network}},
        columns/TotalNum/.style = {column name=$N_T$},
        columns/ConvNum/.style = {column name=\#},
        columns/NumKernels/.style = {column name= $n_l\times n_k$},
        columns/SzKernels/.style = {column name= size},
        columns/ConvOutDims/.style = {column name= output dim},
        columns/FCNum/.style = {column name=\#},
        columns/FCSize/.style = {column name=$n_h$ per layer},
        columns/OutputType/.style = {column name=function},
        columns/OutputNum/.style = {column name=$n_o$},
        col sep=&,
        row sep=\\
    }
}
\begin{table}[b]
\setlength{\tabcolsep}{4.2pt}
  \caption{\textbf{Deep Networks of Different Width:} Size details of deep ConvNet (16 layer) with different widths used in our experiments.}
  \label{tab:network_size}
\centering
{\centering
  \pgfplotstabletypeset[NetworkParams]{ 
    network & TotalNum & NumKernels & ConvOutDims & FCNum &
    FCSize %% & OutputType & OutputNum
    \\
    Deep Tiny  & 21M & 13$\times$64 & 8$\times$8$\times$64 & 3 & (4096, 4096, 1000)     \\
    \midrule
    Deep Small  & 43M &13$\times$128& 8$\times$8$\times$128& 3 & (4096, 4096, 1000)     \\
    \midrule
    Deep Med  & 89M &13$\times$256& 8$\times$8$\times$256& 3 & (4096, 4096, 1000)     \\
  }
}
\\[2pt]
\raggedright
{\footnotesize{ 
Refer to the caption of Table \ref{tab:network_size} for explanation on notation used in this table. All convolutional kernels spatial size is 3x3.}}
\label{tab:net_sizes_depth}
\end{table}

